FastTextSpotter: A High-Efficiency Transformer for Multilingual Scene Text Spotting

The proliferation of scene text in both structured and unstructured environments presents significant challenges in optical character recognition (OCR), necessitating more efficient and robust text spotting solutions. This paper presents FastTextSpotter, a framework that integrates a Swin Transformer visual backbone with a Transformer Encoder-Decoder architecture, enhanced by a novel, faster self-attention unit, SAC2, to improve processing speeds while maintaining accuracy. FastTextSpotter has been validated across multiple datasets, including ICDAR2015 for regular texts and CTW1500 and TotalText for arbitrary-shaped texts, benchmarking against current state-of-the-art models. Our results indicate that FastTextSpotter not only achieves superior accuracy in detecting and recognizing multilingual scene text (English and Vietnamese) but also improves model efficiency, thereby setting new benchmarks in the field. This study underscores the potential of advanced transformer architectures in improving the adaptability and speed of text spotting applications in diverse real-world settings. The dataset, code, and pre-trained models have been released in our Github.

==> tex/rebuttal.tex <==
We sincerely thank the reviewers for their time.  Before addressing their concerns, we shortly summarize the strengths of the paper as identified by Reviewer \textbf{{\color{blue}{R1}}} for highlighting ``The integration of the Swin Transformer backbone with the Transformer Encoder-Decoder architecture and the novel SAC2 attention unit shows a high level of innovation, enhancing both efficiency and accuracy in text spotting tasks. The model is thoroughly evaluated on multiple datasets, including regular and arbitrary-shaped texts, demonstrating its robustness and generalizability. Besides, the paper effectively addresses multilingual text spotting, including low-resource languages like Vietnamese, highlighting its broader applicability. FastTextSpotter sets new benchmarks in terms of operational efficiency, achieving higher frames per second (FPS) compared to state-of-the-art models``; Reviewer \textbf{\color{magenta}{R2}} for highlighting ``The model performance is strong, able to beat 2023 SOTAs. Besides, the inference cost is also slow.  Although the technical contribution of the submission from my point of view is limited, a stack of existing techniques and result in a good performance is also worthy. This paper is also well written and easy-to-follow.``; Reviewer \textbf{\color{teal}{R3}} for recommending ``The proposed method is interesting and the paper is well structured and easy to follow. The paper thoroughly evaluates FastTextSpotter across multiple datasets, validating the model's performance in diverse scenarios. The proposed model outperforms the SOTA systems in the text detection task: in the recall metric for the Total-Text and CTW1500 datasets, in the precision metric for the CTW1500 and ICDAR-15 datasets; and in the text recognition task: in the end-to-end ‘Full’ evaluation of CTW1500 and in the h-mean metric for the Vintext dataset.
The study of ablation and the examples throughout the article help the reader to understand the contribution of each component of the architecture.``.


\noindent\textbf{Q:({\color{blue}{R1}})} Error Analysis and Robustness: There is a lack of detailed error analysis and discussion on the robustness of the model under challenging conditions. Providing a thorough analysis of failure cases, such as handling occlusions, varying lighting conditions, and highly distorted text, would help in understanding the limitations and areas for improvement.

\noindent\textbf{Q:({\color{blue}{R1}})}  Limited Language Scope: While the paper addresses English and Vietnamese, it would benefit from a broader evaluation on more diverse languages and scripts to further validate its multilingual capabilities.

\noindent\textbf{Q: (\textbf{\color{magenta}{R2}})} Only a PDF is provided in the supplementary material. As mentioned above, the value of the submission is a public resource that can be shared in the OCR field. Therefore, the authors should prepare a github repo includes off-the-shied resources

\noindent\textbf{Q: (\textbf{\color{magenta}{R2}})} The authors argue that their method supports multilingual scene text. However, only two languages are evaluated. The authors should include more languages like Chinese, Korean, Japanese, Indian, French etc.

\noindent\textbf{Q:({\textbf{\color{teal}{R3}}})} The improvement of the convergence efficiency of the SAC2 unit, depicted in Figure 1, does not seem significant. More details are needed to reach a clear conclusion.

\noindent\textbf{Q:({\textbf{\color{teal}{R3}}})} The evaluation protocol is missing, which makes it difficult to interpret the metrics and results. It is not clear what metrics are used for text recognition for Total-Text, CTW1500 and ICDAR-15 and what the authors consider to be accurate detection in the case of the text detection task for these datasets.

\noindent\textbf{Q:({\textbf{\color{teal}{R3}}})} The interpretation of the FPS metric is unclear. The claim that the method shows optimal performance in terms of FPS is questionable, as the MANGO system outperforms the model proposed by the authors, if assuming that a lower FPS is better. In the case where higher FPS is better, most of the SOTA systems outperform the proposed model.

\newpage


